Resource-constrained knowledge diffusion processes inspired by human peer learning

We consider a setting where a population of artificial learners is given, and the objective is to optimize aggregate measures of performance, under constraints on training resources. The problem is motivated by the study of peer learning in human educational systems. In this context, we study natural knowledge diffusion processes in networks of interacting artificial learners. By `natural', we mean processes that reflect human peer learning where the students' internal state and learning process is mostly opaque, and the main degree of freedom lies in the formation of peer learning groups by a coordinator who can potentially evaluate the learners before assigning them to peer groups. Among else, we empirically show that such processes indeed make effective use of the training resources, and enable the design of modular neural models that have the capacity to generalize without being prone to overfitting noisy labels.

==> Figures/Forward_Operations/GCN/Pretrain/fig.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.45\textwidth]{Figures/Forward_Operations/GCN/Pretrain/BTB.png}
\includegraphics[width=0.45\textwidth]{Figures/Forward_Operations/GCN/Pretrain/EQ.png}
\includegraphics[width=0.45\textwidth]{Figures/Forward_Operations/GCN/Pretrain/RGBT.png}
\includegraphics[width=0.45\textwidth]{Figures/Forward_Operations/GCN/Pretrain/OO.png}
\caption{Forward Operations for GCN}
\label{fig:forward-gcn}
\end{figure*}




==> Figures/Forward_Operations/Lenet/Pretrain/fig.tex <==
\begin{figure*}[f]
     \centering
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Forward_Operations/Lenet/Pretrain/BTB.png}
         \caption{\scriptsize \textit{BTB}}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Forward_Operations/Lenet/Pretrain/EQ.png}
         \caption{\scriptsize \textit{EQ}}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Forward_Operations/Lenet/Pretrain/RGBT.png}
         \caption{\scriptsize \textit{RGBT}}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Forward_Operations/Lenet/Pretrain/OO.png}
         \caption{\scriptsize \textit{OO}}
     \end{subfigure}
        \caption{Forward Operations for Lenet}
        \label{fig:forward-lenet}
\end{figure*}

==> Figures/Forward_Operations/Resnet/Pretrain/fig.tex <==
\begin{figure*}[f]
     \centering
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Forward_Operations/Resnet/Pretrain/BTB.png}
         \caption{\scriptsize \textit{BTB}}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Forward_Operations/Resnet/Pretrain/EQ.png}
         \caption{\scriptsize \textit{EQ}}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Forward_Operations/Resnet/Pretrain/RGBT.png}
         \caption{\scriptsize \textit{RGBT}}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Forward_Operations/Resnet/Pretrain/OO.png}
         \caption{\scriptsize \textit{OO}}
     \end{subfigure}
        \caption{Forward Operations for Resnet}
        \label{fig:forward-resnet}
\end{figure*}

==> Figures/Forward_Operations/figg.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.32\textwidth]{Figures/Forward_Operations/Lenet/Pretrain/BTB.png}
\includegraphics[width=0.32\textwidth]{Figures/Forward_Operations/Resnet/Pretrain/BTB.png}
\includegraphics[width=0.32\textwidth]{Figures/Forward_Operations/GCN/Pretrain/BTB.png}

\includegraphics[width=0.32\textwidth]{Figures/Forward_Operations/Lenet/Pretrain/EQ.png}
\includegraphics[width=0.32\textwidth]{Figures/Forward_Operations/Resnet/Pretrain/EQ.png}
\includegraphics[width=0.32\textwidth]{Figures/Forward_Operations/GCN/Pretrain/EQ.png}


\includegraphics[width=0.32\textwidth]{Figures/Forward_Operations/Lenet/Pretrain/RGBT.png}
\includegraphics[width=0.32\textwidth]{Figures/Forward_Operations/Resnet/Pretrain/RGBT.png}
\includegraphics[width=0.32\textwidth]{Figures/Forward_Operations/GCN/Pretrain/RGBT.png}


\includegraphics[width=0.32\textwidth]{Figures/Forward_Operations/Lenet/Pretrain/OO.png}
\includegraphics[width=0.32\textwidth]{Figures/Forward_Operations/Resnet/Pretrain/OO.png}
\includegraphics[width=0.32\textwidth]{Figures/Forward_Operations/GCN/Pretrain/OO.png}

\caption{Ensemble accuracy $acc_{\cal E}$ on test set as a function of number of \textit{Forward Operations}. As expected, Split-In-Two out performs Split-In-Five, since it makes 4X higher use of the training set}
\label{fig:forward-gcn}
\end{figure*}



==> Figures/Forward_Operations/figg15_to_7.tex <==
\begin{figure}[h]
     \centering
     \begin{subfigure}
         \centering
         \includegraphics[width=42mm]{Figures/Forward_Operations/Lenet/Pretrain/BTB.png}
         % \caption{\scriptsize LeNet}
     \end{subfigure}     
     \begin{subfigure}
         \centering
        \includegraphics[width=42mm]{Figures/Forward_Operations/Resnet/Pretrain/BTB.png}
         % \caption{\scriptsize ResNet}
     \end{subfigure}
    \caption{Ensemble accuracy $acc_{\cal E}$ on test set as a function of number of \textit{Forward Operations} for LeNet and ResNet. As expected, Split-In-Two out performs Split-In-Five, since it makes 4X higher use of the training set}
    \label{fig:forward-lenet-resent}
\end{figure}




==> Figures/Ground_Truth_Access/GCN/Pretrain/fig.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.42\textwidth]{Figures/Ground_Truth_Access/GCN/Pretrain/BTB.png}
\includegraphics[width=0.42\textwidth]{Figures/Ground_Truth_Access/GCN/Pretrain/EQ.png}\\
\includegraphics[width=0.42\textwidth]{Figures/Ground_Truth_Access/GCN/Pretrain/RGBT.png}
\includegraphics[width=0.42\textwidth]{Figures/Ground_Truth_Access/GCN/Pretrain/OO.png}
    \caption{Ensemble accuracy $acc_{\cal E}$ on test set as a function of the number $\alpha$ of oracle sessions, for \textit{C=2}, \textit{C=5}.}
\label{fig:ground-truth-gcn}
\end{figure*}




==> Figures/Ground_Truth_Access/Lenet/Pretrain/fig.tex <==
\begin{figure*}[f]
     \centering
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Ground_Truth_Access/Lenet/Pretrain/BTB.png}
         \caption{\scriptsize \textit{BTB}}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Ground_Truth_Access/Lenet/Pretrain/EQ.png}
         \caption{\scriptsize \textit{EQ}}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Ground_Truth_Access/Lenet/Pretrain/RGBT.png}
         \caption{\scriptsize \textit{RGBT}}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Ground_Truth_Access/Lenet/Pretrain/OO.png}
         \caption{\scriptsize \textit{OO}}
     \end{subfigure}
        \caption{}
        \label{fig:groun-truth-lenet}
\end{figure*}

==> Figures/Ground_Truth_Access/Resnet/Pretrain/fig.tex <==
\begin{figure*}[f]
     \centering
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Ground_Truth_Access/Resnet/Pretrain/BTB.png}
         \caption{\scriptsize \textit{BTB}}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Ground_Truth_Access/Resnet/Pretrain/EQ.png}
         \caption{\scriptsize \textit{EQ}}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Ground_Truth_Access/Resnet/Pretrain/RGBT.png}
         \caption{\scriptsize \textit{RGBT}}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Ground_Truth_Access/Resnet/Pretrain/OO.png}
         \caption{\scriptsize \textit{OO}}
     \end{subfigure}
        \caption{Ground Truth Access for Resnet}
        \label{fig:ground-truth-resnet}
\end{figure*}

==> Figures/Ground_Truth_Access/figg.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.3\textwidth]{Figures/Ground_Truth_Access/Lenet/Pretrain/EQ.png}
\includegraphics[width=0.3\textwidth]{Figures/Ground_Truth_Access/Lenet/Pretrain/RGBT.png}
\includegraphics[width=0.3\textwidth]{Figures/Ground_Truth_Access/Lenet/Pretrain/OO.png}
\includegraphics[width=0.3\textwidth]{Figures/Ground_Truth_Access/Resnet/Pretrain/EQ.png}
\includegraphics[width=0.3\textwidth]{Figures/Ground_Truth_Access/Resnet/Pretrain/OO.png}
\includegraphics[width=0.3\textwidth]{Figures/Ground_Truth_Access/Resnet/Pretrain/RGBT.png}
\caption{Ensemble accuracy $acc_{\cal E}$ on test set as a function of the number $\alpha$ of oracle sessions, for \textit{C=2} and \textit{C=5}. Figures for \textit{EQ}, \textit{RGBT} and \textit{OO} are shown here, results for \textit{BTB} can be found in \textit{Training Resource Utilization} section.}
\label{fig:groun-truth-lenet}
\end{figure*}




==> Figures/average_no_pretrain.tex <==
\begin{figure*}[]
\centering
\includegraphics[width=0.3\textwidth]{Figures/Average_no_pretrain/Lenet_Paired_shaded.png}
\includegraphics[width=0.3\textwidth]{Figures/Average_no_pretrain/ResNet_Paired_shaded.png}
\includegraphics[width=0.3\textwidth]{Figures/Average_no_pretrain/GCN_Paired_shaded.png}
\includegraphics[width=0.3\textwidth]{Figures/Average_no_pretrain/Lenet_Star_shaded.png}
\includegraphics[width=0.3\textwidth]{Figures/Average_no_pretrain/ResNet_Star_shaded.png}
 \includegraphics[width=0.3\textwidth]{Figures/Average_no_pretrain/GCN_Star_shaded.png}
\caption{Average Learner Accuracy $alacc_{\cal E}$ on test set for 10 rounds/epochs \textbf{without pre-training}. \\ Above:  Split-in-Five $(C=2)$ grouping. Below: Split-in-Two $(C=5)$. \\ Comment: $alacc_{\cal E}$ is higher for higher $acc_{\cal E}$. Note that the reported metrics are averages over multiple random experiments, as discussed in Section~\ref{sec:results}. Coordinated Policies (i.e. {\em BTB} and {\em EQ}) outperform other policies.}
\label{fig:average_no_pretrain} 
\end{figure*}


==> Figures/average_pretrain.tex <==
% \begin{figure*}[]
%      \centering
%      \begin{subfigure}{0.29\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/Average_pretrain/Lenet_Paired.png}
%          \caption{\scriptsize Lenet}
%      \end{subfigure}
%      \begin{subfigure}{0.29\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/Average_pretrain/ResNet_Paired.png}
%          \caption{\scriptsize ResNet}
%      \end{subfigure}
%      \begin{subfigure}{0.29\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/Average_pretrain/GCN_Paired.png}
%          \caption{\scriptsize GCN}
%      \end{subfigure}
%      \begin{subfigure}{0.29\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/Average_pretrain/Lenet_Star.png}
%          \caption{\scriptsize Lenet}
%      \end{subfigure}
%      \begin{subfigure}{0.29\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/Average_pretrain/ResNet_Star.png}
%          \caption{\scriptsize ResNet}
%      \end{subfigure}
%      \begin{subfigure}{0.29\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/Average_pretrain/GCN_Star.png}
%          \caption{\scriptsize GCN}
%      \end{subfigure}
%         \caption{Average Learner Accuracy $alacc_{\cal E}$ on test set for 10 rounds/epochs \textbf{with pre-training}. \\ Above:  Split-in-Five $(C=2)$ grouping. Below: Split-in-Two $(C=5)$. \\ Comment: $alacc_{\cal E}$ is higher for higher $acc_{\cal E}$. Note that the reported metrics are averages over multiple random experiments, as discussed in Section~\ref{sec:setting}. Policy {\em BTB} appears to outperform on LeNet and GCN. However the moderately coordinate {\em RGBT} outperforms on ResNet. Note that ResNet is a much bigger and deeper model that already reaches very high accuracy after round 1. This may suggest that Random Grouping policies may be better for later stages of learning. It is also worth studying ResNet in a setting with more granular rounds, as discussed in Section~\ref{sec:open}. }
%         \label{fig:average_pretrain}
% \end{figure*}



\begin{figure*}[h]
    \centering
    \subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Average_pretrain/Lenet_Paired.png}} 
    \subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Average_pretrain/ResNet_Paired.png}} 
    \subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Average_pretrain/GCN_Paired.png}} 
    \subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Average_pretrain/Lenet_Star.png}} 
    \subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Average_pretrain/ResNet_Star.png}} 
    \subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Average_pretrain/GCN_Star.png}} 
    \caption{Average Learner Accuracy $alacc_{\cal E}$ on test set for 10 rounds/epochs \textbf{with pre-training}. \\ Above:  Split-in-Five $(C=2)$ grouping. Below: Split-in-Two $(C=5)$. \\ \textbf{Comment:} $alacc_{\cal E}$ is higher for higher $acc_{\cal E}$. Note that the reported metrics are averages over multiple random experiments, as discussed in Section~\ref{sec:setting}. Policy {\em BTB} appears to outperform on LeNet and GCN. However the moderately coordinate {\em RGBT} outperforms on ResNet. Note that ResNet is a much bigger and deeper model that already reaches very high accuracy after round 1. This may suggest that Random Grouping policies may be better for later stages of learning. It is also worth studying ResNet in a setting with more granular rounds, as discussed in Section~\ref{sec:open}.}
   \label{fig:average_pretrain}
\end{figure*}

==> Figures/ensemble_no_pretrain.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.30\textwidth]{Figures/Ensemble_no_pretrain/Lenet_Paired_shaded.png}
\includegraphics[width=0.30\textwidth]{Figures/Ensemble_no_pretrain/ResNet_Paired_shaded.png}
\includegraphics[width=0.30\textwidth]{Figures/Ensemble_no_pretrain/GCN_Paired_shaded.png}
\includegraphics[width=0.30\textwidth]{Figures/Ensemble_no_pretrain/GCN_Paired_shaded.png}
\includegraphics[width=0.30\textwidth]{Figures/Ensemble_no_pretrain/ResNet_Star_shaded.png}
\includegraphics[width=0.30\textwidth]{Figures/Ensemble_no_pretrain/GCN_Star_shaded.png}
\caption{Ensemble Accuracy $acc_{\cal E}$ on test set for 10 rounds/epochs \textbf{without pre-training}. \\ Above:  Split-in-Five $(C=2)$ grouping. Below: Split-in-Two $(C=5)$. \\ Comment: $acc_{\cal E}$ is higher for higher $C$.  Note that the reported metrics are averages over multiple random experiments, as discussed in Section~\ref{sec:results}. {\em OO} outperforms only on ResNet. Highly-coordinate policies {\em BTG, EQ} are slighly better than the moderately coordinated {\em RGBT}.}
\label{fig:ensemble_no_pretrain}
\end{figure*}


==> Figures/ensemble_pretrain.tex <==
% \begin{figure*}[]
%      \centering
%      \begin{subfigure}{0.29\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/Ensemble_pretrain/Lenet_Paired.png}
%          \caption{\scriptsize Lenet}
%      \end{subfigure}
%      \begin{subfigure}{0.29\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/Ensemble_pretrain/ResNet_Paired.png}
%          \caption{\scriptsize ResNet}
%      \end{subfigure}
%      \begin{subfigure}{0.29\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/Ensemble_pretrain/GCN_Paired.png}
%          \caption{\scriptsize GCN}
%      \end{subfigure}
%      \begin{subfigure}{0.29\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/Ensemble_pretrain/Lenet_Star.png}
%          \caption{\scriptsize Lenet}
%      \end{subfigure}
%      \begin{subfigure}{0.29\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/Ensemble_pretrain/ResNet_Star.png}
%          \caption{\scriptsize ResNet}
%      \end{subfigure}
%      \begin{subfigure}{0.29\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/Ensemble_pretrain/GCN_Star.png}
%          \caption{\scriptsize GCN}
%      \end{subfigure}
%         \caption{Ensemble Accuracy $acc_{\cal E}$ on test set for 10 rounds/epochs \textbf{with pre-training}. \\ Above:  Split-in-Five $(C=2)$ grouping. Below: Split-in-Two $(C=5)$. \\ Comment: $acc_{\cal E}$ is higher for higher $C$.  Note that the reported metrics are averages over multiple random experiments, as discussed in Section~\ref{sec:setting}. Policy {\em BTB} appears to outperform.}
%         \label{fig:ensemble_pretrain}
% \end{figure*}


\begin{figure*}[h!]
    \centering
    \subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Ensemble_pretrain/Lenet_Paired.png}} 
    \subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Ensemble_pretrain/ResNet_Paired.png}} 
    \subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Ensemble_pretrain/GCN_Paired.png}} 
    \subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Ensemble_pretrain/Lenet_Star.png}} 
    \subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Ensemble_pretrain/ResNet_Star.png}} 
    \subfigure[]{\includegraphics[width=0.32\textwidth]{Figures/Ensemble_pretrain/GCN_Star.png}} 
    \caption{Ensemble Accuracy $acc_{\cal E}$ on test set for 10 rounds/epochs \textbf{with pre-training}. \\ Above:  Split-in-Five $(C=2)$ grouping. Below: Split-in-Two $(C=5)$. \\ \textbf{ Comment:} $acc_{\cal E}$ is higher for higher $C$.  Note that the reported metrics are averages over multiple random experiments, as discussed in Section~\ref{sec:setting}. Policy {\em BTB} appears to outperform.}
    \label{fig:ensemble_pretrain}
\end{figure*}
